A Targeted Sampling Strategy for Compressive Cryo Focused Ion Beam Scanning Electron Microscopy

Cryo Focused Ion-Beam Scanning Electron Microscopy (cryo FIB-SEM) enables three-dimensional and nanoscale imaging of biological specimens via a slice and view mechanism. The FIB-SEM experiments are, however, limited by a slow (typically, several hours) acquisition process and the high electron doses imposed on the beam sensitive specimen can cause damage. In this work, we present a compressive sensing variant of cryo FIB-SEM capable of reducing the operational electron dose and increasing speed. We propose two Targeted Sampling (TS) strategies that leverage the reconstructed image of the previous sample layer as a prior for designing the next subsampling mask. Our image recovery is based on a blind Bayesian dictionary learning approach, i.e., Beta Process Factor Analysis (BPFA). This method is experimentally viable due to our ultra-fast GPU-based implementation of BPFA. Simulations on artificial compressive FIB-SEM measurements validate the success of proposed methods: the operational electron dose can be reduced by up to 20 times. These methods have large implications for the cryo FIB-SEM community, in which the imaging of beam sensitive biological materials without beam damage is crucial.

==> Compressive Cryo FIB Scanning Electron Microscopy (arxiv)/packages.tex <==
\usepackage{amssymb,amsthm,amsmath,array}
\usepackage[top=1in, left=1in, right=1in, bottom=1in]{geometry}
\usepackage{graphicx}
\usepackage[caption=false,font=footnotesize]{subfig}
\usepackage{xspace}
\usepackage[sort&compress, numbers]{natbib}
\usepackage{stmaryrd}
\usepackage{xcolor}
\usepackage{todonotes}
\usepackage{mathtools}
\usepackage{float}
\usepackage{textcomp}

%\usepackage{standalone}
\graphicspath{{Figures/}}

%% TIKS
\usepackage{tikz}
% To boost compilation time with TIKZ
\usetikzlibrary{external}
\tikzexternalize % activate!
%% end of boosting
\usetikzlibrary{arrows}
\usepackage{pgfplots}
\pgfplotsset{compat=1.7}

% special font
\newcommand{\fs}{\mathsf}
\newcommand{\cc}{\centering}
\newcommand{\bs}{\boldsymbol}
\newcommand{\bb}{\mathbb}
\newcommand{\cl}{\mathcal}

% New Theorems
\newtheorem{thm}{Theorem}
\newtheorem{lem}{Lemma}
\newtheorem{prop}{Proposition}
\newtheorem{cor}{Corollary}
\newtheorem{definition}{Definition}
\newtheorem{remark}{Remark}

% Misc
\newcommand{\ts}{\textstyle}
\newcommand{\ie}{\emph{i.e.},\xspace}
\newcommand{\eg}{\emph{e.g.},\xspace}
\newcommand{\etal}{\emph{et al.}}
\newcommand{\sq}{\vspace{-2mm}}

%% Comments
\newcommand{\AMc}[1]{\textcolor{blue}{\small\textbf{[AM: #1]}}}
\newcommand{\ARc}[1]{\textcolor{red}{\small\textbf{[AR: #1]}}}
\newcommand{\JWc}[1]{\textcolor{orange}{\small\textbf{[JW: #1]}}}
\newcommand{\DNc}[1]{\textcolor{magenta}{\small\textbf{[DN: #1]}}}

\renewenvironment{abstract}{\bf {\em\ Abstract---}}{}

\makeatletter
\renewcommand{\section}{\@startsection {section}{1}{\z@}%
             {-3.5ex \@plus -1ex \@minus -.2ex}%
             {2.3ex \@plus.2ex}%
             {\normalfont\large\bfseries}}
\makeatother
